A Geometric Characterization of the Symmetrized Bidisc

The symmetrized bidisc \[ G \stackrel{\rm{def}}{=}\{(z+w,zw):|z|<1,\ |w|<1\} \] has interesting geometric properties. While it has a plentiful supply of complex geodesics and of automorphisms, there is nevertheless a unique complex geodesic $\mathcal{R}$ in $G$ that is invariant under all automorphisms of $G$. Moreover, $G$ is foliated by those complex geodesics that meet $\mathcal{R}$ in one point and have nontrivial stabilizer. We prove that these properties, together with two further geometric hypotheses on the action of the automorphism group of $G$, characterize the symmetrized bidisc in the class of complex manifolds.

==> charactautos.tex <==

\section{Characterization of $G$ via its automorphism group} \label{charactautos}
For a domain  $\Omega$ we denote by $\aut\Omega$ the group of biholomorphic mappings of $\Omega$ onto $\Omega$. In this section we shall show how, for a domain $\Omega$ in $\c^2$, various geometric conditions on the action of $\aut\Omega$ on $\Omega$  lead to criteria for $\Omega$ to be biholomorphic to $G$.




$\aut\Omega$ carries a natural topology, the {\em compact-open topology}, with respect to which it is a topological group.  This topology is defined to be the coarsest topology containing all sets of the form
\beq\label{defKO}
U_\Omega(K,O) \df \{g\in\aut\Omega:g(K) \subset O\},
\eeq
where $K$ is compact and $O$ is open in $\Omega$.   A theorem of H. Cartan \cite{cartan} states that if $\Omega$ is irreducible then $\aut\Omega$ is a Lie group and the group action $(\aut\Omega) \times \Omega \to \Omega$ is a real-analytic map of real manifolds.

\subsection{The action of $\aut \d$ on $G$}

\black
Every automorphism $m$ of $\d$ induces a map $\gamma_m:G \to G$ via the formula
\be\label{aut10}
\gamma_m (\lambda^1+\lambda^2,\lambda^1\lambda^2) = (m(\lambda^1)+m(\lambda^2),m(\lambda^1)m(\lambda^2))
\ee
for $\la^1,\la^2 \in\d$.
It is easy to check that this formula defines a map $\gamma_m \in G(G)$ and that $\gamma_m \in \aut  G$.
\begin{prop} \label{gamiso}
 The map $\Theta:\aut \d \to \aut  G$ given by
\be\label{aut20}
 \Theta(m) = \gamma_m 
\ee
for $m\in\aut \d$ is a continuous isomorphism of topological groups.
\end{prop}


\begin{proof}  The fact that $\Theta$ is an isomorphism of groups is proved in \cite[Theorem 5.1]{AY08} or \cite{jp}.  
We shall show that $\Theta$ is continuous.

We shall denote by $\Gamma$ the closed symmetrised bidisc 
\[
\pi(\overline{\d^2}) = \{(z+w,zw): |z|\leq 1, \, |w|\leq 1\}
\]
and by $t\cdot\Ga$ the compact set
\[
t\cdot\Ga=\pi(t\overline{\d^2}) = \{(z+w,zw): |z|\leq t, \, |w|\leq t\}
\]
for $t>0$.

Observe that a base for the topology of $\aut\d$ is furnished by the sets of the form
\[
U_\d(t\bar\d,O) \quad \mbox{ for } t\in (0,1) \mbox{ and } O\mbox{ open in } \d.
\]
Similarly, the sets 
\[
U_G(t\cdot\Ga,O) \quad \mbox{ where } t\in (0,1) \mbox{ and } O\mbox{ is open in } G
\]
constitute a base for the topology of $\aut G$.

Consider a basic open set $U_G(t\cdot \Ga,O)$ in $\aut G$ for some $t\in (0,1)$ and open subset $O$ of $G$.  For any $m\in\aut\d$,
\begin{align}
\Theta(m) \in U_G(t\cdot\Ga,O) & \Leftrightarrow \ga_m\circ\pi (z,w) \in O \mbox{ for all } z,w \in t\bar \d  \notag \\
	 & \Leftrightarrow \pi(m(z),m(w))  \in O \mbox{ for all } z,w \in t\bar \d  \notag \\
	 & \Leftrightarrow m(t\bar\d) \times m(t\bar\d)\subset \pi\inv(O). \label{1.1}
\end{align}

Consider any point $m_0\in\aut\d$ and any basic open set $U_G(t\cdot\Ga,O)$ of $\Theta(m_0)$.  By the statement \eqref{1.1},
\be\label{1.1a}
m_0(t\bar\d) \times m_0(t\bar\d)\subset \pi\inv(O).
\ee
The following lemma is evident.

{\em  If $C$ is a compact subset of $\d$ and $W$ is an open neighborhood of $C\times C$ in $\d^2$ then there is an open
neighborhood $V$ of $C$ in $\d$ such that $V\times V \subset W$.}  

It follows from equation \eqref{1.1a} that there exists an open neighborhood $V$ of $m_0(t\bar\d)$ in $\d$ such that $\pi(V\times V) \subset O$.  Clearly $N \df U_\d(t\bar\d,V)$ is an open neighborhood of $m_0$ in $\aut\d$ such that 
$\Theta(N) \subset U_G(t\cdot\Ga,O)$. Hence $\Theta$ is continuous at $m_0$.
\end{proof}
\begin{remark}\label{Thetahomeo} \rm
In fact $\Theta:\aut\d\to\aut G$ is not only continuous, it is a homeomorphism.  This statement (which we shall not use) follows from Remark \ref{ctyThetainv} below.
\end{remark}

Let us state precisely the theorem of Cartan \cite{cartan} on continuous transformation groups mentioned above.  (In fact Cartan's statement is more general than the following.)   Let $\Omega$ be a domain in $\c^d$.   A topological group $A$ is said to {\em act continuously} on $\Omega$ if a continuous homomorphism $\Phi: A\to \aut\Omega$ is given.  The pair $(A,\Phi)$ is called a {\em continuous transformation group} on $\Omega$.  The theorem states:

{\em If $(A,\Phi)$ is a continuous transformation group on $\Omega$, $A$ is locally compact, $\Phi$ is injective and $\Omega$ is irreducible, then $A$ is a Lie group and the map $A\times \Omega \to \Omega$ given by $(g,\la)\mapsto \Phi(g)(\la)$ is real-analytic.}

Here is an immediate consequence.
\begin{prop}\label{diffeval}
\begin{enumerate}[(1)]
\item $\aut\d$ and $\aut G$ are Lie groups.
\item For any $s\in G$ the map $F_s:\aut\d\to G$ given by $F_s(m)=\ga_m(s)$ is differentiable.
\end{enumerate}
\end{prop}


\black
\subsection{The action of $\aut G$ on the royal variety}
The {\em royal variety} or {\em royal geodesic} in $G$ is defined to be the set
\begin{align*}
\calr  &= \{s\in G: (s^1)^2=4s^2\} \\
	&=\{(2z,z^2):z\in\d\}.
\end{align*}
Thus  $\calr=R(\d)$ where 
\be\label{aut42}
R(z) = (2z,z^2)\qquad \mbox{ for } z\in \d.
\ee
Clearly
\be\label{aut44}
\gamma_m (R(z)) = R( m (z))\qquad \mbox{ for } z\in \d  \mbox{ and }m\in \aut \d.
\ee

\black
\begin{comment}
\red Simplify the next para \black
How does $\gamma_m$ act on $\calr$?  If $\delta$ is a datum that contacts $\calr$ then the general solution to $\Kob({\delta})$ has the form
\be\label{aut30}
r_b(z) = (2b(z),b(z)^2),\qquad \mbox{ for } z\in \d,
\ee
where $b$ is an element of $\aut (G)$(\textcolor{blue}{reference?}). It then follows from equation \eqref{aut10} that
\be\label{aut40}
\gamma_m (r_b (z)) = r_b\big(b^{-1}\circ m \circ b (z)\big),\qquad z\in \d.
\ee
Thus, if one views $r_b$ as a co-ordinate for $\calr$, then the action of $\gamma_m$ on $\calr$ corresponds to the action of $b^{-1}\circ m \circ b$ on $\d$. In the sequel, we shall set $r=r_b$ in the special case that $b=\id{\d}$. Thus
\be\label{aut42}
r(z) = (2z,z^2),\qquad z\in \d
\ee
and
\be\label{aut44}
\gamma_m (r(z)) = r( m (z)),\qquad z\in \d, \; m\in \aut \d.
\ee
\end{comment}
The observations \eqref{aut20} and \eqref{aut44} have three simple yet striking consequences, summarized in the following proposition.
\begin{prop}\label{autprop10}
\begin{enumerate}[(i)]
\item Every automorphism of $G$ leaves $\calr$ invariant.
\item Every automorphism of $G$ is uniquely determined by its values on $\calr$.
\item Every automorphism of $\calr$ has a unique extension to an automorphism of $G$.
\end{enumerate}
\end{prop}

In statement (iii), automorphisms of $\calr$ are with respect to the structure of $\calr$ as a complex manifold.

We can summarize these three statements by saying that the restriction map $\ga \mapsto \ga|\calr$ is an isomorphism from $\aut  G$ to $\aut\calr$.  The following commutative diagram describes the situation, where $\iota_\calr$ denotes the injection of $\calr$ into $G$ and $m\in\aut \d$.
\be\label{commDiagG}
\begin{array}{rrrcl}
\d & \stackrel{R}{\longrightarrow} &\calr& \stackrel{\iota_\calr}{\longrightarrow} & G \\
\vcenter{\llap{$\scriptstyle{m}$}}\Big\downarrow&  &\vcenter{\llap{$\scriptstyle{\ga_m|\calr}$}}\Big\downarrow & & \vcenter{\llap{$\scriptstyle{\ga_m}$}}\Big\downarrow\\
\d & \stackrel{R}{\longrightarrow} &\calr& \stackrel{\iota_\calr}{\longrightarrow} & G
\end{array}
\ee
\black


\subsection{ Orbits in $G$ as manifolds\black}
For any domain $U$ and any $\lambda \in U$,  let $\orb_U(\lambda)$ denote the orbit of $\lambda$ under the action of the group of automorphisms of $U$:
\[
\orb_U(\lambda) = \set{\gamma(\lambda)}{\gamma \in \aut(U)}.
\]

Consider the case that $U=G$ and $\lambda=s\in G$.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% See  `keepcharactautos.tex' for the text at 12.11.16, before my major adjustments.

In view of Proposition \ref{gamiso}, for any $s\in G$,
\beq\label{formOrbs}
\orb_G(s)=\{\ga_m(s): m\in\aut\d\},
\eeq
and so $\orb_G(s)$ is the range of the action map  $a_s:\aut\d\to G$ where
\be\label{defFs}
a_s(m)= \ga_m(s).
\ee
$\aut\d$ is a real $3$-dimensional manifold, for which we shall need local co-ordinates.
For $(r,\alpha) \in \r \times \d$ let $m_{r,\alpha} \in \aut\d$ be given by the formula
\be\label{aut90}
m_{r,\alpha} (z) =\e^{ir}\frac{z-\alpha}{1-\bar\alpha z}, \qquad z\in\d.
\ee
The automorphisms of $\d$ consist of the maps $m_{r,\al}$ for $r\in\r$ and $\al\in\d$. 
Let
\[
U_1=\{m_{r,\alpha}: -\pi < r<\pi, \, \al\in\d\},  \quad U_2=\{m_{r,\alpha}: 0 < r<2\pi, \, \al\in\d\}.
\]
We have $\aut\d=U_1 \cup U_2$.  Define 
\[
\ph_1:U_1 \to (-\pi,\pi)\times \d \quad \mbox{ by } \quad  \ph_1(m_{r,\alpha})=(r, \al),
\]
and similarly for $\ph_2:U_2\to (0,2\pi)\times \d$.  Then $(U_1,\ph_1)$ and $(U_2,\ph_2)$ are charts in $\aut\d$ which together comprise a $C^\infty$ atlas $\cala$ for the group manifold.  The identity automorphism $\idd=m_{0,0}$ belongs to $U_1$.  
By Cartan's Theorem, $a_s$ is real-analytic  from $(\aut\d,\cala)$ to $\c^2$.  In local co-ordinates, by a straightforward calculation, for any $s\in G,\,  r\in\r$ and $\al\in \d$,
\[
a_s(m_{r,\al})= \frac{\left(\e^{ir}(-2\al+(1+|\al|^2)s^1-2\bar\al s^2), \e^{2ir}(\al^2-\al s^1+s^2)\right)}{1-\bar\al s^1+\bar\al^2 s^2}.
\]






\begin{prop}\label{autrem15} 
If $s \not\in \calr$ then the map  $a_s:\aut\d\to \orb_G(s)$
is a two-to-one covering map and is a local homeomorphism.
\end{prop}


\begin{proof}
Consider a point $s=(z+w,zw)\in G$ where $z,w \in \d$ and $z \neq w$.   Let $\up$ be the unique automorphism of $\d$ that maps 
$z$ to $w$ and $w$ to $z$.  Note that  $ \up$ 
is not the identity automorphism ${\mathrm{id}}_{\d}$ since $z \neq w$.
For $m_1,m_2 \in \aut\d$,
\begin{align}
\ga_{m_1}(s)=\ga_{m_2}(s) & \Leftrightarrow \pi(m_1(z),m_1(w))=\pi(m_2(z),m_2(w)) \notag \\
	&  \Leftrightarrow  \left\{ \begin{array}{l}\mbox{ either } m_1(z)=m_2(z) \mbox{ and } m_1(w)=m_2(w) \\
						\mbox{ or } m_1(z)=m_2(w) \mbox{ and } m_1(w)=m_2(z)  \end{array} \right. \notag\\
	&  \Leftrightarrow  \left\{ \begin{array}{l}\mbox{ either } m_1=m_2 \\
						\mbox{ or } m_2\inv\circ m_1=\up.
						   \end{array} \right. \label{2to1}
\end{align}
  The map $a_s:m \mapsto \ga_m(s)$ is therefore two-to-one from $\aut\d$ to $ \orb_G (s)$.


Since the map $(m_1,m_2) \mapsto {m_2}\inv \circ {m_1}$ is continuous from $\aut \d\times \aut \d$ to $\aut \d$ and maps $(\idd,\idd)$ to $\mathrm{id}_\d$, the set $\{(m_1,m_2): m_2\inv \circ m_1\neq\up\}$ is a neighborhood of $(\idd,\idd)$ in $\aut \d\times \aut \d$.  Hence there exists a neighborhood $U$ of $\idd$ such that 
\beq\label{m1m2}
m_2\inv \circ m_1\neq \up\quad \mbox{  for all } m_1, m_2 \in U.
\eeq
We claim that, for any $\beta\in \aut  G$, the set 
\[
\beta\circ \ga_U \df\{\beta\circ \ga_u: u\in U\}
\]
 is a neighborhood of $\beta$ on which  the evaluation map $E_s: \aut  G \to G$ given by
\[
E_s(\ga)=\ga(s)
\]
is injective.  Certainly it is a neighborhood of $\beta$, and if $E_s|\beta \circ \ga_U$ is not injective then there exist distinct points $m_1,m_2 \in U$ such that $E_s(\beta\circ\ga_{m_1})=E_s(\beta\circ\ga_{m_2})$.  That is, $\beta\circ\ga_{m_1}(s)=\beta\circ\ga_{m_2}(s)$, and therefore $\ga_{m_1}(s)=\ga_{m_2}(s)$.
Hence, by the equivalence \eqref{2to1}, $m_2\inv \circ m_1=\up$.  This equation contradicts the statement \eqref{m1m2}.  Thus $E_s$ is locally injective on $\aut{G}$, and so the map $m \mapsto \ga_m(s)$ is injective from $U\subset\aut \d$ to $\orb_G(s)$.

Choose a compact neighborhood $V$ of $\idd$ contained in $U$.  Since a continuous bijective map from a compact space to a Hausdorff space is a homeomorphism, $a_s|V$ is a homeomorphism onto its range.  It follows by homogeneity that $a_s$ is a local homeomorphism on $\aut\d$.  Indeed, consider any $m\in \aut\d$ and its neighborhood $m(V)$.   Define $L_m:\aut\d\to\aut\d$ by $L_m(\theta)= m\inv\circ\theta$ for $\theta\in\aut\d$. In the commutative diagram
\be\label{commDiagFs}
\begin{array}{rrrcl}
m(V) & \stackrel{a_s|m(V)}{\longrightarrow} &a_s(m(V))\\
\vcenter{\llap{$\scriptstyle{L_m|m(V)}$}}\Big\downarrow&  &\vcenter{\llap{$\scriptstyle{\ga(m)|a_s(V)}$}}\Big\uparrow\\
V & \stackrel{a_s|V}{\longrightarrow} & a_s(V) 
\end{array}
\ee
the map $a_s|m(V)$ is expressed as the composition of three homeomorphisms, and so is itself a homeomorphism.  Thus $a_s$ is a local homeomorphism.
\end{proof}

\begin{thm}\label{autprop30a}
\begin{enumerate}[(1)]
\item If $s \in \calr$, then $\orb_G (s)$ is a one-dimensional complex manifold properly embedded in $G$.  

\item If $s \in G \setminus  \calr$, then 
$\orb_G (s)$ is a three-dimensional real $C^\infty$ manifold properly embedded in $G$.   
\end{enumerate}
Moreover, in either case, the tangent space to $\orb_G(s)$ at $s$ is
\be\label{basisV}
\calv(s) \df \spa_\r\left\{ i\bpm s^1\\2s^2\epm, \bpm 2-(s^1)^2 + 2s^2 \\s^1-s^1s^2 \epm, i\bpm 2 +(s^1)^2 -2s^2 \\ s^1 + s^1s^2 \epm  \right\}.
\ee
\begin{comment}
In both cases
\be\label{aut104}
\calv(s)=T_s \orb_G (s).
\ee
\end{comment}
\end{thm}
Here the notation $T_s\orb_G(s)$ denotes the complex tangent space if $s\in\calr$ and the real tangent space if $s\notin\calr$.
\begin{proof}

Consider $s\in G$. 
We shall calculate the rank of the real linear operator $a_s'(m)$ for $m\in\aut \d$.


Consider a tangent vector $(r,\al)$ at $(0,0)$ to $(-\pi,\pi)\times\d$.  Thus $(r,\al)\in \r\times\c$.  Define a path $\kappa(t)=(tr,t\al)$ in $(-\pi,\pi)\times\d$ for $|t|<\eps$, where $\eps$ is small enough.
\black
Then define $v_{r,\alpha} (s) \in \c^2$ by the formula
\begin{align}
v_{r,\alpha}(s)&=\frac{\dd}{\dd t} a_s\circ \ph_1\inv\circ\kappa(t)\big|_{t=0}\label{defvra}  \\
	&= \frac{\dd}{\dd t} a_s\circ m_{\kappa(t)}\big|_{t=0} \notag \\
	&=\frac{\dd}{\dd t} a_s\circ m_{tr,t\al}\big|_{t=0} \notag \\
	&= \frac{\dd}{\dd t} \ga_{ m_{tr,t\al}}(s)\big|_{t=0}.\label{aut92}
\end{align}
From equation \eqref{aut90}, for any $z\in\d$, 
\[
\frac{\dd}{\dd t} m_{tr,t\alpha} (z) \big|_{t=0} = irz - \alpha +\bar \alpha z^2.
\]

Hence, by equations \eqref{aut10} and \eqref{aut92}, if $s=(z_1+z_2,z_1z_2)$,
\begin {align}\label{aut95}
v_{r,\alpha} (s) &=  \frac{\dd}{\dd t} \left. \bpm m_{tr,t\al}(z_1)+m_{tr,t\al}(z_2) \\ m_{tr,t\al}(z_1) m_{tr,t\al}(z_2) \epm\right|_{t=0} \notag \\
	&= \bpm irz_1-\al+\bar\al(z_1)^2 + irz_2-\al+\bar\al (z_2)^2 \\
		(  irz_1-\al+\bar\al(z_1)^2)z_2 + (irz_2-\al+\bar\al (z_2)^2)z_1 \epm  \notag \\
	&=ir\begin{pmatrix}s^1\\2s^2\end{pmatrix}
	-\alpha\begin{pmatrix}2\\s^1\end{pmatrix}
	+\bar\alpha\begin{pmatrix}{(s^1)}^2-2s^2\\s^1s^2\end{pmatrix}.
\end{align}
Let $f_s=a_s\circ \ph_1\inv$.
By the Chain Rule we also have, from equation \eqref{defvra},
\begin{align}
v_{r,\al}(s) &= f_s'(\kappa(0))\kappa'(0) \notag \\
	&= f_s'(0,0) \bpm r\\  \al\epm. \label{formvra2}
\end{align}
Thus the range of the real linear map $f_s'(0,0): \r\times\c \to \c^2$ is the set
\begin{align*}
\ran f_s'(0,0) &= \{v_{r,\al}: r\in\r, \al\in\c\} \\
	&=\left\{ir\begin{pmatrix}s^1\\2s^2\end{pmatrix}
	-\alpha\begin{pmatrix}2\\s^1\end{pmatrix}
	+\bar\alpha\begin{pmatrix}{(s^1)}^2-2s^2\\s^1s^2\end{pmatrix}:r\in\r, \, \al\in\c\right\}.
\end{align*}
On taking $(r,\al)$ to be successively $(1,0), \, (0,-1)$ and $(0,-i)$ we find that, for any $s\in G$,
\[
\ran f_s'(0,0) = \calv(s),
\]
the real vector space introduced in equation \eqref{basisV}.  Thus
\be\label{rankFs}
\ran a_s'(\idd)=\ran f_s'(0,0) = \calv(s)
\ee
for all $s\in G$.

Now consider $s\in G\setminus \calr$.  
By Lemma \ref{autlem8} below, $\dim_\r \calv(s) = 3$, and so, by equation \eqref{rankFs},
$a_s'(\idd)$ has rank $3$.  We claim that $a_s'(m)$ has rank $3$ for all $m\in \aut \d$.   Indeed, on differentiating the relation
\[
a_s(m)=\ga_m(s)=\ga_m\circ \ga_{\idd}(s)=\ga_m\circ a_s(\idd),
\]
we find (since $a_s(\idd)=s$) that
\[
a_s'(m)= \ga_m'(s)a_s'(\idd).
\]
\red Add a basic ref on diff geom for $a_s'$ \black \\
Since $\ga_m$ is an automorphism of $G$, $\ga_m'(s)$ is a nonsingular real linear transformation of $\c^2$.   Thus
\[
\rank_\r a_s'(m) = \rank_\r a_s'(\idd) =3
\]
for every $m\in\aut\d$.

We wish to deduce that $\orb_G(s)$ is a real $3$-dimensional $C^\infty$-manifold in $\c^2$.
The following statement is \cite[Theorem 5.2]{Spiv}.

 {\em A subset $M$ of $\r^n$ is a $k$-dimensional manifold if and only if, for every point $s\in M$ there exist an open neighborhood $V$ of $s$ in $\r^n$, an open set $W$ in $\r^k$ and an injective differentiable function $f:W \to \r^n$ such that 
\begin{enumerate}[\rm (1)]
\item $f(W)=M\cap V$,
\item $f'(y)$ has rank $k$ for every $y\in W$.
\end{enumerate}
}


We shall apply this criterion in the case $n=4, \ k=3, \ M=\orb_G(s)$.  Choose an open neighborhood $N$ of $\idd$ in $U_1$ such that $a_s|N$ is a homeomorphism from $N$ to an open subset of $\orb_G(s)$.  Then, since $\orb_G(s)$ has the relative topology induced by $G$, there is an open set $V$ in $\r^4$ such that $a_s(N)= V\cap \orb_G(s)$.

Let $W=\ph_1(N)$.  Then the map $f= a_s\circ \ph_1\inv$ satisfies conditions (1) and (2).  It follows that $\orb_G(s)$ is a real $3$-dimensional $C^\infty$ manifold in $\c^2$.

The linear map $(a_s\circ \ph_1\inv)'(0,0)$ maps  the tangent space $T_{(0,0)} (-\pi,\pi)\times\d$ into the tangent space $T_s\orb_G(s)\subset \c^2$.    We have seen that the range of $(a_s\circ \ph_1\inv)'(0,0)$ is $\calv(s)$.  Hence 
\[
\calv(s) \subseteq  T_s\orb_G(s).
\]
Since both spaces have real dimension $3$, the inclusion holds with equality.


In the case that $s\in\calr$, say $s=(2\zeta,\zeta^2)$ for some $\zeta\in\d$,
\[
\orb_G(s)=\calr=\{(2z,z^2): z\in\d\},
\]
 which is  a one-dimensional complex manifold properly embedded in $G$ by the map $R:\d\to G$.
The complex tangent space to $\calr$ at $s$ is $\c(1,\zeta)$, and, by equation \eqref{basisV},
\begin{align*}
\calv(s)&=\spa_\r\left\{ i\zeta\bpm 1 \\ \zeta\epm, (1-\zeta^2)\bpm 1 \\ \zeta \epm, i(1+\zeta^2)\bpm 1 \\ \zeta \epm \right\} \\
	&=\c\bpm 1 \\ \zeta \epm.
\end{align*}
Thus $T_s\orb_G(s) = \calv(s)$ in the sense of complex manifolds.
\end{proof}


\begin{lem}\label{autlem8}
For any $s\in G$, the set
\be\label{aut96}
\calv (s) = \set{v_{r,\alpha} (s)}{r\in \r, \alpha \in \c}
\ee
 is a real subspace of $\c^2$.  Moreover
\be\label{aut100}
\dim_\r  \calv(s) =\left\{ \begin{array}{lll}3 &\quad &\mbox{ if }  (s^1)^2\neq 4 s^2  \\  
								2    &\quad & \mbox{ if }  (s^1)^2 = 4 s^2.  \end{array} 
			    \right.
 \ee
\end{lem}
\red Zina to check \black
%Observe that $\{s: (s^1)^2\overline {s^2}\in\r\}$ is a $3$-dimensional real algebraic variety that contains the royal variety.
\begin{proof}

It is clear from equation \eqref{aut95} that $\calv(s)$ is a real vector subspace of $\c^2$ of real dimension at most $3$.

Suppose that scalars $\la,\mu,\nu \in\r$ satisfy
\be\label{linrel}
\la i\bpm s^1\\2s^2\epm + \mu \bpm 2-(s^1)^2 + 2s^2 \\s^1-s^1s^2 \epm + \nu i\bpm 2 +(s^1)^2 -2s^2 \\ s^1 + s^1s^2 \epm =0.
\ee
Multiply on the left by the row matrix $\bpm 2s^2 & -s^1 \epm$ to obtain
\be\label{elimla1}
-((s^1)^2-4s^2)\left((1+s^2)\mu + (1-s^2)\nu i \right)=0.
\ee
Consider the first case in equation \eqref{aut100}, namely, that  $(s^1)^2\neq 4s^2$ (equivalently,  $s\notin \calr$).  By equation \eqref{elimla1}
\[
(1+s^2)\mu + (1-s^2)\nu i=0,
\]
whence
\[
\mu+i\nu= -s^2(\mu-i\nu).
\]
Since $s\in G$, we have $|s^2|<1$, and so necessarily $\mu=\nu=0$.  Since $(s^1)^2\neq 4s^2$, at least one of
$s^1,s^2$ is nonzero, and so, by equation \eqref{linrel}, $\la=0$.  Hence the three spanning vectors for $\calv(s)$ in equation \eqref{basisV} are linearly independent.  We have shown that $\dim_\r \calv(s) =3$ when $s\notin \calr$.

Next consider a point $s\in \calr$.   On substituting $s^2= \tfrac 14 (s^1)^2$ in equation \eqref{basisV} we obtain
\[
\calv(s)=\spa_\r\left\{ is^1\bpm 2\\ s^1 \epm, (4-(s^1)^2)\bpm 2\\ s^1 \epm, i(4+(s^1)^2) \bpm 2\\ s^1 \epm    \right\}.
\]
Since each of these vectors is a complex scalar multiple of the vector $\bpm 2 & s^1 \epm^T$, it follows that $\dim_\r \calv(s) \leq 2$.


In fact $\dim_\r \calv(s) = 2$.  For otherwise the second and third spanning vectors for $\calv(s)$ are linearly dependent over $\r$, and so there exist $\mu,\nu \in\r$, not both zero, such that
\[
\mu ( 4-(s^1)^2)+\nu i (4+(s^1)^2) = 0
\]
and consequently
\[
4(\mu +\nu i)=(s^1)^2(\mu-\nu i).
\]
Thus $|s^1|=2$, contrary to choice of $s\in G$.
Therefore
\[
\dim_\r \calv(s) = 2 \quad \mbox{ when } s \in\calr.
\]
\end{proof}

\black


\subsection{Royal domains}
Let us say that $D$ is an \emph{analytic disc in a domain $\Omega$} if there exists $k\in \Omega(\d)$ such that $D=\ran k$. If, in addition, $k$ can be chosen to be a \emph{ proper embedding} (that is,  a proper injective analytic mapping with $k'(z)\neq 0$ for all $z\in \d$), then we will say that $D$ is a  \emph{properly embedded analytic disc in $\Omega$}. 

%The set $D$ is said to be an {\em analytic retract} of $\Omega$ if there is an analytic map $\rho:\Omega\to\Omega$ such that $\rho\circ\rho=\rho$ and  $D=\ran\rho$.
\black
\begin{defin}\label{autdef10}
For a domain $\Omega$, we say that $D$ is a \emph{royal disc in $\Omega$} if $D$ is a properly embedded analytic disc in $\Omega$
%\blue $D$ is an analytic retract of $\Omega$  \black
and $D$ satisfies the three properties of Proposition \ref{autprop10}, that is,
\begin{enumerate}[(i)]
\item each automorphism of $\Omega$ leaves $D$ invariant,
\item each automorphism of $\Omega$ is uniquely determined by its values on $D$,
\item each automorphism of $D$ has an extension to an automorphism of $\Omega$.
\end{enumerate}
A \emph{royal domain} is an ordered pair $(\Omega,D)$ where $\Omega$ is a domain in $\c^2$ and $D$ is a royal disc in $\Omega$.
\end{defin}
\blue
Perhaps allow $\Omega$ to be a $2$-dimensional complex manifold?
\black

The following lemma is straightforward. 
%\blue Note that $\calr$ is an analytic retract in $G$: the map  \[ \rho(s)=(s^1, \tfrac 14 (s^1)^2) \]
%is an idempotent analytic map in $G(G)$ with range $\calr$.
\black
\begin{lem}\label{autlem4}
If $\Lambda:G\to \Omega$ is a biholomorphic map, then $\Lambda(\calr)$ is a royal disc in $\Omega$ and $(\Omega, \Lambda(\calr))$ is a royal domain.
\end{lem}
The next proposition spells out the analog of formula \eqref{aut44} on a general royal domain.
\begin{prop}\label{autprop20}
Let $(\Omega,D)$ be a royal domain. Then $\aut\Omega$ is isomorphic to $\aut \d$. Furthermore, if $k:\d \to \Omega$ is a proper embedding such that $k(\d)=D$, then there exists a unique isomorphism $\Theta:\aut \d\to \aut\Omega$ such that
\be\label{aut50}
\Theta(m) \circ k = k\circ m \qquad \mbox{ for all }  m\in \aut \d.
\ee
\end{prop}

The counterpart of the commutative diagram \eqref{commDiagG} is
\be\label{commDiagO}
\begin{array}{rrrcl}
\d & \stackrel{k}{\longrightarrow} &D& \stackrel{\iota_D}{\longrightarrow} & \Omega \\
\vcenter{\llap{$\scriptstyle{m}$}}\Big\downarrow&  &\vcenter{\llap{$\scriptstyle{\Theta(m)|D}$}}\Big\downarrow & & \vcenter{\llap{$\scriptstyle{\Theta(m)}$}}\Big\downarrow\\
\d & \stackrel{k}{\longrightarrow} & D & \stackrel{\iota_D}{\longrightarrow} & \Omega
\end{array}
\ee
where $\iota_D$ is the injection of $D$ into $\Omega$.
\black
\begin{proof}
Fix a proper embedding $k$ such that $k(\d)=D$. For each $\tau \in \aut\Omega$, Condition (i) in Definition \ref{autdef10} implies that there exists a function $\phi_\tau:\d \to \d$ such that
\be\label{aut60}
\tau(k(z)) = k\circ\phi_\tau (z) \qquad \mbox{ for } z \in \d.
\ee
Clearly, since $\tau$ is an automorphism of $\Omega$ and $k$ is a proper embedding, $\phi_\tau \in \aut \d$.

If $\tau_1,\tau_2 \in \aut\Omega$, then for each $z\in \d$ we see using equation \eqref{aut60} that
\begin{align*}
k(\phi_{\tau_2 \circ \tau_1 }(z))&=\tau_2 \circ \tau_1 (k(z))\\
&=\tau_2 ( \tau_1 (k(z)))\\
&=\tau_2(k(\phi_{\tau_1}(z)))\\
&=k(\phi_{\tau_2}(\phi_{\tau_1}(z)))\\
&=k(\phi_{\tau_2}\circ \phi_{\tau_1}(z)).
\end{align*}
This relation proves that the map $\Psi:\aut\Omega \to \aut \d$ given by
\be\label{aut70}
\Psi( \tau)= \phi_\tau
\ee
is a homomorphism of automorphism groups.

If $\tau_1,\tau_2 \in \aut\Omega$ and $\phi_{\tau_1}(z) = \phi_{\tau_2}(z) $ for all $z \in \d$, then equation  \eqref{aut60} implies that $\tau_1(k(z))=\tau_2(k(z))$ for all $z\in \d$, which is to say that $\tau_1$ and $\tau_2$ agree on $D$.  Hence, by Condition (ii) in Definition \ref{autdef10}, $\tau_1=\tau_2$. This proves that $\Psi$ is injective.

Consider any $b\in \aut \d$. As
\[
D \ni k(z) \mapsto k(b(z)) \in D \qquad \mbox{ for } z \in \d
\]
defines an automorphism of the complex manifold $D$, Condition (iii) in Definition \ref{autdef10} implies that there exists $\tau \in \aut\Omega$ such that $\tau(k(z)) = k\circ b(z)$ for all $z\in \d$. But then
\[
k(b(z)) = \tau(k(z)) = k(\phi_\tau(z))
\]
for all $z \in \d$, so that $\phi_\tau = b$. This proves that $\Psi$ is surjective from $\aut\Omega$ onto $\aut \d$.

We have shown that $\Psi$ is an isomorphism of groups. In particular, the first assertion of Proposition \ref{autprop20}  (that $\aut\Omega$ is isomorphic to $\aut \d$) is proven. To define an isomorphism $\Theta$ satisfying the second assertion of the proposition,  let $\Theta  =\Psi\inv$. Then $\Theta$ is an isomorphism from $\aut \d$ onto $\aut\Omega$, and equation \eqref{aut50} follows from the relation \eqref{aut60}.

To see that $\Theta$ is unique fix $m\in \aut \d$ and observe that if $\Theta_1$ and $\Theta_2$ are isomorphisms satisfying equation \eqref{aut60}, then $\Theta_1(m)(k(z))=\Theta_2(m)(k(z))$ for all $z \in \d$. Since $\Theta_1(m) $ and $\Theta_2(m)$ agree on $D$, Condition (ii) in Definition \ref{autdef10} imples that $\Theta_1(m) = \Theta_2(m)$. As $m$ is arbitrary, $\Theta_1=\Theta_2$.
\end{proof}

In the light of Proposition \ref{autprop20} we adopt the following definition.
\begin{defin}\label{autdef15}
Let $(\Omega,D)$ be a royal domain. We say that $(k,\Theta)$ is a \emph{canonical pair for $(\Omega,D)$} if  $k:\d \to \Omega$ is a proper embedding, $k(\d)=D$, and $\Theta:\aut \d\to \aut\Omega$ is an isomorphism satisfying, for all $m\in\aut\d$, 
\[
\Theta(m)\circ k= k\circ m
\]
as in equation \eqref{aut50}.
\end{defin}
  In other words, $(k,\Theta)$ is a canonical pair for $(\Omega,D)$ if the diagram \eqref{commDiagO} commutes for every $m\in\aut \d$.
\begin{remark}\label{autrem10} \rm 
Canonical pairs are essentially unique in the following sense. If $(\Omega,D)$ is a royal domain and $(k_0,\Theta_0)$ is a canonical pair for $(\Omega,D)$, then $(k,\Theta)$ is a canonical pair for $(\Omega,D)$ if and only if there exists $b\in \aut \d$ such that $k=k_0 \circ b$ and $\Theta=\Theta_0 \circ I_b$, where $I_b$ denotes the inner automorphism of $\aut\d$ defined by $I_b (m) = b\circ m \circ b^{-1}$.
\end{remark}

As a companion to Lemma \ref{autlem4} we have the following equally straightforward lemma.
\begin{lem}\label{autlem6}
%As noted in in Lemma \ref{autlem4} 
If $\Lambda:G\to \Omega$ is a biholomorphic map, $k=\Lambda\circ r$ and 
%then $(\Omega,\Lambda(R))$ is a royal domain. If we define $d$ by the formula,
%and if $f, \Ga$ are defined by
%f(z)=\Lambda(r(z)),\qquad \mbox{ for }z\in \d,
%and we define $\Theta$ by the formula,
\be\label{aut80}
\Theta(m) = \Lambda\circ\gamma_m\circ \Lambda^{-1},\qquad \mbox{ for } m \in \aut{\d},
\ee
then $(k,\Theta)$ is a canonical pair for $\Omega$.
\end{lem}

Continuity properties of the isomorphism $\Theta$ appearing in Definition \ref{autdef15} will be important in the sequel.  
We make two observations about continuity.
\begin{remark}\label{autrem11} \rm 
 If $(\Omega,D)$ is a royal domain and $(k,\Theta)$ is a canonical pair for $(\Omega,D)$ and $D$ is an analytic retract in $\Omega$, then $k$ has an analytic left inverse.  For we may choose an idempotent $\rho\in\Omega(\Omega)$ such that $\ran\rho=D$; then $\Phi\df k\inv\circ \rho\in \d(\Omega)$ and $\Phi\circ k=\idd$.  It follows from  equation \eqref{aut50} that 
\beq\label{Fthetak}
\Phi\circ \Theta(m)\circ k=m :\d\to\d \quad \mbox{ for all } m\in\aut\d.
\eeq
\end{remark}
\begin{remark}\label{ctyThetainv} \rm
 If $(\Omega,D)$ is a royal domain, $(k,\Theta)$ is a canonical pair for $(\Omega,D)$ and $D$ is an analytic retract in $\Omega$, then $\Theta\inv$ is a continuous map from $\aut\Omega$ to $\aut\d$.
\end{remark}
\begin{proof}
Consider any point $g_0 \in\aut\Omega$ and any basic neighborhood $U_\d(K,O)$ of $\Theta\inv(g_0)$ in $\aut\d$, where $K,O$ are compact and open respectively in $\d$.  By equation \eqref{Fthetak},
\[
\Phi\circ g \circ k= \Theta\inv(g) \quad \mbox{ for all } g\in\aut\Omega.
\]
By choice of $K$ and $O$,
\[
\Theta\inv(g_0)(K) \subset O,
\]
and therefore
\[
\Phi\circ g_0 \circ k(K) \subset O.
\]
It follows that, if 
\[
N \df U_\Omega(k(K), \Phi\inv(O)),
\]
then $g_0\in N$.
That is, $N$ is a basic open neighborhood of $g_0$ in $\aut\Omega$.  If $g\in N$ then
\[
\Phi\circ g\circ k(K) \subset O,
\]
which is to say that
\[
\Theta\inv(g) \in U_\d(K,O).
\]
Therefore
\[
\Theta\inv(N) \subset U_\d(K,O).
\]
Hence $\Theta\inv$ is continuous on $\aut\Omega$.

\end{proof}


\begin{comment}
The next two results will enable us to show that $\Theta$ is continuous for any royal domain.
\begin{lem}\label{compcts}
The composition map $\Omega(\Omega) \times \Omega(\Omega) \to \Omega(\Omega)$ is continuous for the compact-open topology.
\end{lem}
\begin{proof} \red Omit this \black
Consider $f_0,g_0 \in\Omega(\Omega)$.  We prove that the map $(f,g)\mapsto f\circ g$ is continuous at $(f_0,g_0)$.
Consider a basic neighborhood $U(K,O)\df \{f: f(K)\subset O\}$ of $f_0\circ g_0$ in $\Omega(\Omega)$, where $K,O$ are compact and open respectively in $\Omega$.  Then $f_0\circ g_0(K)\subset O$, and so $g_0(K)\subset f_0\inv(O)$.  Choose an open neighborhood $O_1$ of $g_0(K)$ such that $\overline{O_1}$ is compact and
\[
g_0(K) \subset O_1\subset \overline{O_1} \subset f_1\inv(O).
\]
Now if $f\in U(\overline{O_1},O)$ and $g\in U(K, O_1)$ then
\[
g(K)\subset O_1 \subset \overline{O_1},
\]
and so $f\circ g(K)\subset O$.  Hence $U(\overline{O_1},O)\times U(K, O_1)$ is a neighborhood of $(f_0,g_0)$ whose image under composition is contained in $U(K,O)$.  Thus composition is continuous at $(f_0,g_0)$.
\end{proof}
\end{comment}
\begin{lem}
Let $\Omega$ be a connected taut domain.  If $(h_n)$ is a sequence in $\Omega(\Omega)$ converging to $h\in\bar\Omega(\Omega)$ then $h(\Omega)$ lies either in $\Omega$ or in $\partial\Omega$.
\end{lem}
\begin{proof}
Suppose not. Then $h\inv(\Omega)$ is a nonempty proper open subset of $\Omega$, and so its closure in $\Omega$ contains a point $\la_1 \notin h\inv(\Omega)$. Choose an open ball  $B$ centered at $\la_1$ contained in $\Omega$.  Then  $B$ contains a point $\la_2\in h\inv(\Omega)$ and an analytic disc $D$ such that $\la_1, \la_2 \in D$.  We have $h(\la_1) \in \partial\Omega$ and $h(\la_2)\in\Omega$.  However, $(h_n|D)$ is a sequence of analytic maps from the disc to $\Omega$, and so by tautness, the sequence either has a subsequence that converges locally uniformly in $\Omega(\d)$ (in which case $h(D)\subset \Omega$) or diverges locally uniformly on $D$ (in which case $h(D) \subset \partial\Omega$).  This is a contradiction.
\end{proof}
\begin{prop}\label{Thcts}
Let $(\Omega,D)$ be a royal domain and let $(k,\Theta)$ be an associated canonical pair.    If $\Omega$ is taut and $\aut\Omega$ is locally bounded on $\Omega$, then the map $\Theta:\aut\d\to\aut\Omega$ is continuous.
\end{prop}
\begin{proof}
  The compact-open topology on  $\aut\Omega$, which is the same as the topology of locally uniform convergence, is metrizable.  It therefore suffices to prove the sequential continuity of $\Theta$.

Consider a sequence $(m_n)$ in $\aut\d$ converging to $\idd$.  Note that, for any $\la\in D$, say $\la=k(z)$ where $z\in\d$,
\be\label{fixD}
\Theta(m_n)(\la)=\Theta(m_n)\circ k(z)= k\circ m_n(z) \to k(z)=\la \quad \mbox{ as } n\to \infty.
\ee
Since $\aut\Omega$ is locally bounded,  Montel's Theorem applies to the sequence $(\Theta(m_n))$ in $\Omega(\Omega)$ to show that the sequence either has a subsequence that converges to an element of $\Omega(\Omega)$ or has a subsequence that diverges locally uniformly on $\Omega$.  Statement \eqref{fixD} rules out the second alternative, and so, after passage to a subsequence, we may assume that $\Theta(m_n)$ converges to a function $h\in\Omega(\Omega)$ which fixes every point of $D$.  Similarly, after passage to a further subsequence, we may suppose that $\Theta(m_n)\inv$ converges to some function $g\in \Omega(\Omega)$.  Since the composition map $(h,g)\mapsto h\circ g$ is continuous for the compact-open topology,
\[
\id{\Omega}= \lim_{n\to\infty} \Theta(m_n)\circ \Theta(m_n)\inv = h\circ g.
\]
Likewise $g\circ h=\id{\Omega}$.  Thus $h\in\aut\Omega$.    Since $h$ acts as the identity automorphism on $D$, it follows from property (ii) of Definition \ref{autdef10} that $h=\id{\Omega}$.  We have shown that $\Theta$ is continuous at $\id{\d}$.  It follows easily that $\Theta$ is continuous at every point of $\aut\d$.
\end{proof}
\blue
\begin{corollary}\label{isobdd}
If $(k,\Theta)$ is a canonical pair for a royal domain $(\Omega,D)$, where $\Omega$ is a taut connected domain that is isomorphic to a bounded domain, then $\Theta$ is continuous.
\end{corollary}
\begin{proof}
Suppose $\Lambda:\Omega\to \Omega_1$ is a biholomorphic map and $\Omega_1$ is a bounded domain.  Then $(\Omega_1,\Lambda(D))$ is a royal domain for which $(\Lambda\circ k, \Theta_1)$ is a canonical pair, where $\Theta_1(m)= \Lambda\circ\Theta(m)\circ\Lambda\inv$ for every $m\in\aut\d$.  Since $\Omega_1$ is a bounded connected taut domain, $\Theta_1$ is continuous by Proposition  \ref{Thcts}.  Therefore $\Theta(\cdot)= \Lambda\inv\circ\Theta_1(\cdot)\circ\Lambda$ is continuous.
\end{proof}
\red
I still don't know whether $\Theta$ is always continuous.  It would be good to have a counterexample if not.
\black

\subsection{Regularity properties of royal domains}
\begin{comment}
For the extension of these notions to a general royal domain $(\Omega,D)$ it is desirable that the orbits $\orb_\Omega (s)$ be smooth manifolds. In particular, we want the analog of the vector $v_{r,\alpha} (s)$ in the last subsection to be well defined. We therefore formulate a definition.
\red    Note first that, according to Cartan's Theorem,  $\aut\Omega$ is a Lie group and the action $(\aut \Omega)\times\Omega \to \Omega$ is a real-analytic map of real manifolds.  {\em A fortiori,}
for any $\la\in\Omega$, the evaluation map $E_\la: \aut\Omega \to \c^2$ given by
\beq\label{defEla}
E_\la(\ga)=\ga(\la) \quad \mbox{ for } \ga\in\aut\Omega
\eeq
 is a differentiable map of real manifolds.  We introduce the notation
\beq\label{defWla}
\calw(\la)=\ran E_\la'(\mathrm{id}_\Omega) \quad \mbox{ for } \la\in\Omega.
\eeq
Thus $\calw(\la)$ is a real subspace of the real tangent space $T_\la\c^2$.
\end{comment}

\begin{defin}\label{autdef24}
Let $(\Omega,D)$ be a royal domain and $(k,\Theta)$ a corresponding canonical pair. We say that $(\Omega,D)$ is \emph{regular} if $\Theta$ is continuous and, for every $\lambda\in \Omega \setminus D$,
\be\label{aut110}
\rank_\r e_\lambda'(\idd) =3
\ee
where $e_\la:\aut\d\to \Omega$ is defined by $e_\la (m)=\Theta(m)(\la)$.
\end{defin}
By Cartan's Theorem,  $e_\la$ is real-analytic.  The map
$e_\la'(\idd)$ is a linear mapping between real tangent spaces,
\[
e_\la'(\idd): T_{\idd}\aut\d \to T_\la\Omega.
\] 
Clearly continuity of $\Theta$
 does not depend on the particular canonical pair $(k,\Theta)$ for $(\Omega,D)$.
\begin{remark}\label{autrem40} \rm
The natural analog of equation \eqref{aut100}, to wit, 
\[
\rank_\r e_\lambda'(\idd) =2 \quad \mbox{  if }\lambda\in D,
\]
 is not required in  Definition \ref{autdef24}, since the condition holds automatically, as is clear from the following statement.
\end{remark}

\black
\begin{prop}\label{autprop35}
Let $(\Omega,D)$ be a regular royal domain. 
\begin{enumerate}[(1)]
\item  If $\lambda\in D$ then $\orb_\Omega (\lambda)$ is a one-dimensional complex manifold properly embedded in $\Omega$.  
\item  If $\lambda \in \Omega\setminus  D$, then $\orb_\Omega (\lambda)$ is a three-dimensional real manifold properly embedded in $\Omega$. 
\end{enumerate}
In both cases
\be\label{aut112}
\ran e_\lambda'(\idd)=T_\lambda \orb_\Omega (\lambda)
\ee

in the sense of complex or real tangent spaces, as appropriate.
\end{prop}

\begin{proof}
\blue
Let $(k,\Theta)$ be a canonical pair for $\Omega$ and let $k=(k^1,k^2):\d\to\Omega$.

(1)  Let $\la\in D$.  By conditions (i) and (iii) in Definition \ref{autdef10}, $\orb_\Omega(\la) = D$, which is by hypothesis a properly embedded analytic disc in $\Omega$. 

Consider a point $\la\in D$, so that  $\la=k(z)$ for some $z\in\d$. A routine calculation shows the following.  There exists a nonzero vector $v\in T_\la\Omega$ such that, for every tangent vector $\de$ to $\aut\d$ at $\idd$,
\be\label{striking}
e_\la'(\idd)\de = \ip{\ev_z}{ \de_\c} v
\ee
where $\ev_z:\aut\d \to\d$ is the evaluation function
\[
\ev_z(m) = m(z) \quad \mbox{ for } m\in\aut\d
\]
and $\de_\c$ denotes the complexification of $\de$, so that, for any complex-valued $C^1$ function $h$ in a neighborhood of $\idd$,
\[
\ip{h}{\de_\c}= \ip{\re h}{\de}+i\ip{\im h}{\de}.
\]
In fact, in terms of the real variables $x^1,y^1,x^2,y^2$, where points of $\Omega$ are written as $(z^1,z^2)=(x^1+iy^1,x^2+iy^2)$,
\begin{align}\label{defv}
v&=\re {k^1}'(z)\frac{\partial}{\partial x^1}{\left|_\la\right.} + \im { k^1}'(z)\frac{\partial}{\partial y^1}\left|_\la\right. +
	\re {k^2}'(z)\frac{\partial}{\partial x^2}\left|_\la\right. + \im  {k^2}'(z)\frac{\partial}{\partial y^2}\left|_\la\right. \\
	&= 2\re\left\{{k^1}'(z)\frac{\partial}{\partial z^1}\left|_\la\right.  + {k^2}'(z) \frac{\partial}{\partial z^2} \left|_\la\right. \right\} \notag
\end{align}
where, as usual,
\[
\frac{\partial }{\partial z^j} = \frac{1}{2}\left( \frac{\partial}{\partial x^j}-i  \frac{\partial}{\partial y^j}\right).
\]
Since $k$ is by hypothesis a proper embedding, $k'(z)\neq 0$, and therefore $v\neq 0$.

It is immediate from equation \eqref{striking} that $\rank_\r e_\la'(\idd)$ is at most $2$.  To show it is at least $2$ one can calculate $\ip{\ev_z}{ \de_\c}$ in local co-ordinates $r,\al$ as in equation \eqref{aut90}, or better, $r,\xi,\eta \in\r$ where $\al=\xi+i\eta$.  One finds that if
\[
\de= \de_1\frac{\partial}{\partial r}+\de_2 \frac{\partial}{\partial \xi}+\de_3 \frac{\partial}{\partial \eta} \quad \mbox{ at } z,
\]
where $\de_1,\de_2,\de_3 \in\r$, then 
\[
\ip{\ev_z}{\de_\c} = iz\de_1 + (z^2-1)\de_2 -i(z^2+1) \de_3.
\]
Since $|z|<1$, the vectors $z^2-1$ and $-i(z^2+1)$ are linearly independent in the real vector space $\c$, and so
\[
\{\ip{\ev_z}{\de_\c}: \de \in T_{\idd}\aut\d\}=\c.
\]
Hence 
\[
\ran e_\la'(\idd) = \c v
\]
and $\rank_\r  e_\la'(\idd) =2$, as claimed.
\end{proof}

\black
A comparison of formulas \eqref{aut92} and \eqref{aut106} allows one to set up a linear correspondence between the spaces $\calv$ and $\calw$ defined in \eqref{aut96} and \eqref{aut108} respectively. Explicitly, for fixed $s\in G$ and $\lambda \in \Omega$ we define the real linear mapping
\[
\frac{d\Gamma}{d\gamma}:\calv(s) \to \calw(\lambda)
\]
by the formula
\be\label{aut114}
\frac{d\Gamma}{d\gamma} ( v_{r,\alpha}) = w_{r,\alpha},\qquad r\in \r,\alpha\in \c.
\ee
Note here, that the notation has suppressed the dependence of $d\Gamma/d\gamma$ on $s$ and $\lambda$. In the sequel, when this is an issue, we shall employ the somewhat clugey expression
\[
\big(\frac{d\Gamma}{d\gamma}\big)_{s,\lambda}.
\]
\subsection{The action of $\aut  G$ on flat geodesics}
The flat geodesics in $G$ have a special role to play in the hyperbolic geometry of $G$. There is a rich theory of these geodesics (\textcolor {blue}{reference}). We recall the following facts from this theory:
\begin{enumerate}
\item Through each point $s$ in $G$ there passes a unique flat geodesic $F_s$.
\item Each flat geodesic intersects the royal geodesic in exactly one point.
\item Automorphisms of $G$ carry flat geodesics to flat geodesics.
\end{enumerate}

\noindent The following lemma is just a reformulation of the first two of these facts.
\begin{lem}\label{autlem10}
If we define $\calf$ by
\[
\calf = \set{F_s}{s \in R}
\]
then $\calf$ is a partition of $G$.
\end{lem}

\noindent Also, these facts imply the following concrete description of the action of $\aut  G$ on $\calf$.
\begin{lem}\label{autlem20}
If $\gamma \in \aut  G$ and $s\in R$, then $\gamma (F_s) = F_{\gamma(s)}$.
\end{lem}
\begin{proof}
Fix $\gamma \in \aut  G$ and $s\in R$. By Fact 3, there exists $t\in R$ such that $\gamma(F_s) =F_t$, and Condition (i) in Proposition \ref{autprop10} implies that $\gamma(s) \in R$. Therefore we have that
$t, \gamma(s) \in R\cap F_t$. Hence by Fact 2,  $t=\gamma(s)$.
\end{proof}
\subsection{Flat fibrations over royal discs}
In this section we shall formalize the structure laid out in the previous subsection.
\begin{defin}\label{autdef30}
Let $(\Omega,D)$ be a royal domain. If $\cale =\set{E_\lambda}{ \lambda\in D}$ is a family of sets indexed by $D$, then we say that $\cale$ is a \emph{flat fibration of $\Omega$ over $D$} if
\begin{enumerate}[(i)]
\item For each $\lambda \in D$, $E_\lambda$ is a properly embedded analytic disc in $\Omega$,
\item $\cale$ is a partition of $\Omega$ (cf. Lemma \ref{autlem10}), and
\item if $\Gamma \in \aut\Omega$ and $\lambda\in D$, then $\Gamma (E_\lambda) = E_{\Gamma(\lambda)}$. (cf. Lemma \ref{autlem20}).
\end{enumerate}
We say that $(\Omega,D,\cale)$ is a \emph{flatly fibered royal domain} if $(\Omega,D)$ is a royal domain and $\cale$ is a flat fibration of $\Omega$ over $D$.
\end{defin}

\begin{lem}\label{autlem24}
As noted in Lemma \ref{autlem6}, if $\Lambda:G \to \Omega$ is a biholomorphic map, then $(\Omega,\Lambda(\d)$ is a royal domain and $(d, \Gamma)$, as defined in the lemma, is a canonical pair for $(\Omega,\Lambda(\d))$. If, in addition, we let $\cale =\set{E_{d(z)}}{z \in \d}$ where for each $z\in \d$ we define $E_{d(z)}$ by
\[
E_{d(z)} = \Lambda (F_{r(z)}),
\]
then $\cale$ is flat fibration of $\Omega$ over $D$ and $(\Omega,\Lambda(\d),\cale)$ is a flatly fibered royal domain.
\end{lem}
\begin{comment}
\begin{prop}\label{autprop30}
Let $\Lambda:G \to \Omega$ be a biholomorphic mapping.  Let $d=\Lambda \circ r$ and $D=\Lambda(\d)$. For each $\lambda=\Lambda(s) \in D$, define $E_\lambda$ by $E_d = \Lambda(F_s)$ and then set $\cale=\set{E_\lambda}{\lambda \in D}$. Then $D$ is a royal disc in $G$ and $(d, \cale)$ is a flat fibration over $D$ that is compatible with $G$ at each point $d_0 \in D$.
\end{prop}
\end{comment}
 \subsection{Synchronicity}
Fix $s_0 \in R$. Then $R$ and $F_{s_0}$ are embedded analytic discs in $G$ that intersect transversally at the point $s_0$. Furthermore, if $\gamma\in \aut_{s_0} (G)$, the stabilizer of $s_0$,  then $\gamma$ is an automorphism of $R \cup F_{s_0}$. In general, for such an automorphism there need be no connection between the action on the two leaves $R$ and $F_0$ beyond what is implied by the condition $(\gamma|R) (s_0) = s_0 =( \gamma|F_{s_0})(s_0)$. However, in the current situation, in light of Condition (ii) in Proposition \ref{autprop10} the action of $\gamma$ on $F_{s_0}$ is uniquely determined by the action of $\gamma$ on $R$. The following lemmas describe this dependence explicitly.
\begin{lem}\label{autlem30}
If $s_0\in R$ and $\gamma\in \aut_{s_0} (G)$, then $d\gamma _{s_0}$ has eigenspaces $T_{s_0} R$ and $T_{s_0}F_{s_0}$ with corresponding eigenvectors $\eta$ and $\eta^2$ for some $\eta\in \t$.
\end{lem}
\begin{proof}
For $\eta \in \t$ let $\rho_\eta$ denote the element of $\aut \d$ defined by $\rho_\eta(z) = \eta z$. Let $s_0=r(z_0)$. Since $\gamma\in \aut_{s_0} (G)$, $\gamma=\gamma_m$ where $m(z_0)=z_0$. Therefore, there exists $\eta\in \t$ such that
\[
m= b_{-z_0} \circ \rho_\eta \circ b_{-z_0}^{-1}
\]
which implies that
\[
\gamma = \gamma_{b_{-z_0}} \circ \gamma_{\rho_\eta} \circ \gamma_{b_{-z_0}}^{-1}.
\]
It follows by the chain rule that
\[
d\gamma_{s_0} = X (d\gamma_{\rho_\eta})_{(0,0)}X^{-1}
\]
Where $X=(d\gamma_{b_{-z_0}})_{(0,0)}$. But
\[
(d\gamma_{\rho_\eta})_{(0,0)}=\begin{bmatrix}\eta & 0\\ 0& \eta^2\end{bmatrix}
\]
has eigenspaces $\c \oplus 0$ and $0 \oplus \c$ with corresponding eienvectors $\eta$ and $\eta^2$. Therefore, $d\gamma _{s_0}$ has eigenspaces $X (\c \oplus 0)$ and $X(0 \oplus \c)$ with corresponding eigenvectors $\eta$ and $\eta^2$. That $X (\c \oplus 0) = T_{s_0} R$ and $X(0 \oplus \c)=T_{s_0}F_{s_0}$ follows either by direct calculation or by noticing that $R$ and $F_{s_0}$ are invariant for $\gamma$.
\end{proof}
\begin{lem}\label{autlem40}
Let $s_0=r(z_0)$ and $\gamma\in \aut_{s_0} G$. Choose $m\in \aut \d$ so that $\gamma=\gamma_m$. If $f$ is any proper embedding of $\d$ into $G$ with $f(\d) =F_{s_0}$ and $f(z_0)=s_0$, then
\[
\gamma(f(z)) = f((m\circ m) (z))
\]
\end{lem}
\begin{proof}
Note that since $\gamma\in \aut_{s_0} G$, $m(z_0) =z_0$, and  also that,
\[
\gamma(r(z)) = r(m(z))
\]
for all $z\in \d$. This equation implies that
\[
d\gamma_{s_0} r'(z_0) =m'(z_0) r'(z_0),
\]
i.e., $m'(z_0)$ is the eigenvalue of $d\gamma_{s_0}$ corresponding to the eigenspace $T_{s_0} R$. Consequently, by Lemma \ref{autlem30},
\footnotesize
\be\label{aut116}
m'(z_0)^2 \text{ is the eigenvalue of  } d\gamma_{s_0} \text{ corresponding to the eigenspace } T_{s_0} F_{s_0}.
\ee
\normalsize

Now, since $f$ is a proper embedding and $\gamma (F_{s_0}) = F_{s_0}$, there exists $b \in \aut{\d}$ such that
\[
\gamma(f(z)) = f(b(z))
\]
for all $z\in \d$. Noting that $b(z_0)=z_0$, this equation implies that
\[
d\gamma_{s_0} f'(z_0) =b'(z_0) f'(z_0),
\]
i.e., $b'(z_0)$ is the eigenvalue of $d\gamma_{s_0}$ corresponding to the eigenspace $T_{s_0} F_{s_0}$. Therefore, statement \eqref{aut116} implies that
\[
b'(z_0) =m'(z_0)^2 = (m\circ m)'(z_0),
\]
Since $b,m\circ m \in \aut \d$, $b(z_0) = z_0 = (m \circ m)(z_0)$, and $b'(z_0) = (m\circ m)'(z_0)$, it follows that $b=m\circ m$.
\end{proof}
Lemma \ref{autlem40} suggests the following definition.
\begin{defin}\label{autdef31}
Let $(\Omega,D,\cale)$ be a flatly fibered royal domain with canonical pair $(d,\Gamma)$.  Let $d_0 =d(z_0)$ and choose an embedding $e:\d \to \Omega$ with $e(\d) = E_{d_0}$ and $e(z_0) = d_0$. We say that \emph{$(\Omega,D,\cale)$ is synchronous with $G$ at $d_0$} if
\[
\Gamma(m)(e(z)) =e((m \circ m) (z))
\]
for all $z \in \d$ and all $m\in \aut_{z_0} \d$.
\end{defin}
\begin{remark}\label{autrem50}
If $(\Omega,D,\cale)$ is as in the definition, then the synchronicity of $(\Omega,D,\cale)$ with $G$ at $d_0$ depends neither on the choice of $(d,\Gamma)$ nor the choice of $e$.
\end{remark}
\begin{remark}\label{autrem60}
If $(\Omega,D,\cale)$ is as in the definition, then $(\Omega,D,\cale)$ is synchronous with $G$ at a particular $d_0\in D$ if and only if $(\Omega,D,\cale)$ is synchronous with $G$ at $\lambda$ for every $\lambda\in D$. Consequently, it makes sense to say simply that \emph{$(\Omega,D,\cale)$ synchronous with $G$}.
\end{remark}
\begin{lem}\label{autlem44}
If $(\Omega,D,\cale)$ is as in Lemma \ref{autlem24}, then $(\Omega,D,\cale$ is synchronous with $G$.
\end{lem}
\subsection{Linearity in the sharp direction}
In the event that $s\in G\setminus R$ and Lemma \ref{autlem8} guarantees that $\calv(s)$ is a 3 real dimensional subspace of $\c^2$, $\calv(s)$ contains a unique 2 real dimensional subspace that is also a one dimensional complex subspace. We denote this space with $s^\sharp$ and refer to it as the \emph{sharp direction}.  If $s\in R$ we again define the sharp direction by setting $s^\sharp= T_s R$. Clearly, in both cases,
\[
s^\sharp = \calv(s) \cap i\calv(s).
\]
The sharp direction is intrinsically invariant in the sense of the following proposition.
\begin{prop}\label{autprop40}
If $\gamma \in \aut  G$ and $s\in G$, then $(d\gamma)_s (s^\sharp) = (\gamma (s))^\sharp$.
\end{prop}


For a regular royal domain $(\Omega,D)$ we may define the sharp direction just as in $G$. Specifically, for $\lambda \in \Omega$ we set
\[
\lambda^\sharp = T_\lambda \orb_\Omega (\lambda) \cap iT_\lambda \orb_\Omega (\lambda).
\]


The following proposition is proved exactly as Proposition \ref{autprop40} was.
\begin{prop}\label{autprop50}
If $\Gamma\in \aut\Omega$ and $\lambda \in \Omega$, then
\[
\big(d\,  \Gamma \big)_\lambda (\lambda^\sharp) = (\Gamma ( \lambda ) )^\sharp
\]
\end{prop}
Now, let $\Lambda:G \to \Omega$ be a biholomorphic map so that $(\Omega,\Lambda(\d))$ is a royal domain with canonical pair $(d,\Gamma)$ as defined in Lemma \ref{autlem6}. Fix $s\in G$ and $\lambda\in \Omega$ with $\Lambda(s) = \lambda$. If $r\in \r$ and $\alpha \in \c$, then
\begin{align*}
&\ \ \ \ d\Lambda (v_{r,\alpha} (s))\\
\eqref{aut92}\qquad\qquad &= d\Lambda \big(\frac{d}{dt}\gamma_{m_{r,\alpha} (t)} (s) |_{t=0}\big)\\
\text{chain rule}\qquad\qquad &=\frac{d}{dt}\ \big(\Lambda \circ \gamma_{m_{r,\alpha} (t)}\big) (s)\ \big|_{t=0}\\
\eqref{aut80}\qquad\qquad &=\frac{d}{dt}\ \big(\Gamma (m_{r,\alpha} (t))\circ \Lambda \big) (s)\ \big|_{t=0}\\
&= \frac{d}{dt}( \Gamma(m_{r,\alpha} (t))(\lambda))\big|_{t=0}\\
\eqref{aut106}\qquad\qquad &=w_{r,\alpha}(\lambda)\\
\eqref{aut114}\qquad\qquad &=\frac{d\Gamma}{d\gamma}(v_{r,\alpha}(s)),
\end{align*}
i.e.,
\be\label{aut118}
\frac{d\Gamma}{d\gamma} = d\Lambda \big| \calv(s).
\ee
This formula has two implications which we record in the following lemmas.
\begin{lem}\label{autlem50}
If $\Lambda:G \to \Omega$ is a biholomorphic map with $\Lambda(s) =\lambda$ and $(d,\Gamma)$ is the canonical pair of Lemma \ref{autlem6}, then $d\Lambda(\calv(s))=\calw(\lambda)$ and $d\Lambda(s^\sharp) = \lambda^\sharp$.
\end{lem}
\begin{proof}
By \eqref{aut114}, $(d\Gamma/d\gamma) (\calv(s))=\calw(\lambda)$. Therefore, \eqref{aut118} implies that $d\Lambda(\calv(s))=\calw(\lambda)$. Since $d\Lambda$ is invertible and complex linear, and $s^\sharp$ and $\lambda^\sharp$ are the nonzero complex subspaces of $\calv(s)$ and $\calw(\lambda)$ respectively, it follows that $d\Lambda(s^\sharp) = \lambda^\sharp$.
\end{proof}
\begin{lem}\label{autlem60}
If $\Lambda:G \to \Omega$ is a biholomorphic map with $\Lambda(s) =\lambda$ and $(d,\Gamma)$ is the canonical pair of Lemma \ref{autlem6}, then
\be\label{aut120}
\frac{d\Gamma}{d\gamma}(s^\sharp) = \lambda^\sharp.
\ee
Furthermore, $(d\Gamma/ d\gamma) \big| s^\sharp$ is complex linear.
\end{lem}
\textcolor{blue}{
\begin{defin}\label{}
$\Gamma$ acts linearly in the sharp direction on $E_0$ if
\[
f(z)^\sharp\cap\calv(f(z)) \ni v_{r,\alpha} (s) \mapsto w_{r,\alpha} \in e(z)^\sharp \cap \calw(e(z))
\]
is complex linear for each $z \in \d$.
\end{defin}
}
\subsection{Sharpness of the action of $\aut\Omega$}
Fix a regular flatly fibered royal domain $(\Omega,D,\cale)$. In this section we shall formulate a condition that is necessary for $\Omega$ to be biholomorphically equivalent to $G$. In the next subsection we shall show that the condition is also necessary.

Assume that $\Lambda:G \to \Omega$ is biholomorphic. By Lemma \ref{autlem44} it follows that
\be\label{autlem122}
(\Omega,D,\cale) \text{ is synchronous with } G.
\ee

A second necessary condition follows by exploiting equation \eqref{aut120}. Fix a canonical pair $(d,\Gamma)$ and a point $d_0\in D$. We then make the following sequence of constructions.
\begin{enumerate}
\item Choose $z_0\in \d$ so that $d(z_0)=d_0$.
\item Choose an embedding $e:\d \to \Omega$ such that $e(z_0)=d_0$ and $e(\d)=E_{d_0}$.
    \item Set $s_0=r(z_0)$
\item Choose an embedding $f:\d \to G$ such that $f(z_0)=s_0$ and $f(\d)=F_{s_0}$.
\end{enumerate}
With these constructions we observe that $\Lambda$ can be replaced with a new biholomorphic map $\Lambda^\sim:G \to \Omega$ satisfying
$\Lambda^\sim \circ f =e$. But then \eqref{aut120} implies that
\be\label{aut124}
\forall_{z\in \d}\ \ \big(\frac{d\Gamma}{d\gamma}\big)_{f(z),e(z)} (e(z)^\sharp) = f(z)^\sharp.
\ee
This prompts the following definition.
\begin{defin}\label{autdef40}
Let $(\Omega,D,\cale)$ be a regular flatly fibered royal domain with canonical pair $(d,\Gamma)$ and fix $d_0 \in D$. We say that \emph{$\Gamma$ acts sharply over $d_0$} if \eqref{aut124} holds.
\end{defin}
\begin{remark}\label{autrem70}
Needless to say, $\Gamma$ acts sharply over $d_0$ for some $d_0\in D$ if and only if $\Gamma$ acts sharply over $d$ for every $d\in D$. Also, the sharpness condition does not depend on the choice of canonical pair $(d,\Gamma)$. Consequently, the sharpness condition depends only on the action of $\aut\Omega$ on $\Omega$. For this reason we say \emph{$\aut\Omega$ acts sharply on $\Omega$} when the conditions of Definition \ref{autdef40} hold.
\end{remark}
We summarize the results of this section in the following proposition.
\begin{prop}\label{autprop60}
If $\Omega$ is a domain and $\Lambda:G\to \Omega$ is a biholomorphic map then there exist a royal disc $D$ in $\Omega$ and a flat fibration $\cale$ of $\Omega$ over $D$. Furthermore, $(\Omega,D,\cale)$ is regular, synchronous with $G$, and $\aut{\Omega}$ acts sharply on $\Omega$.
\end{prop}
\subsection{A characterization of $G$}
\begin{prop}\label{autprop70}
If $(\Omega,D,\cale)$ is a regular flatly fibered royal domain, synchronous with $G$ and with $\aut{\Omega}$ acts sharply on $\Omega$, then $\Omega$ is biholomorphically equivalent to $G$.
\end{prop}
\begin{proof}
Fix $z_0 \in \d$. We shall construct a biholomorphic map $\Lambda:G \to \Omega$ satisfying $\Lambda(s_0) = d_0$ where $s_0=r(z_0)$.

Fix a proper embedding of $\d$ into $G$ satisfying $f(\d) = F_{s_0}$ and $f(z_0) =s_0$ and let $(d,\Gamma)$ be a canonical pair. Also, fix a proper embedding $e:\d \to \Omega$ with $e(z_0) = d_0$ and $e(\d) = E_{d_0}$. For $s\in G$ we define $\Lambda(s)$ using the following recipe.  Choose $z\in \d$ and $m \in \aut \d$ so that
\be\label{}
s=\gamma_m(f(z))
\ee
and then let
\be\label{aut130}
\Lambda(s)=\Gamma(m)(e(z))
\ee
Since each point in $G$ is in a flat geodesic and $\aut  G$ acts transitively on the royal geodesic, that there exist $z$ and $m$ satisfying \eqref{aut120} follows from Lemma \ref{autlem20}.

To see that this recipe defining $\Lambda$ is well defined, assume that $z_1,z_2 \in \d$, $m_1,m_2 \in \aut \d$, and
\be\label{aut140}
\gamma_{m_1}(f(z_1)) = \gamma_{m_2}(f(z_2)).
\ee
We wish to show that
\be\label{aut150}
\Gamma(m_1)(e(z_1))=\Gamma(m_2)(e(z_2)).
\ee
Note first that \eqref{aut140} implies that if we set $ m=m_2^{-1}\circ m_1 $, then $\gamma_m(f(z_1))=f(z_2)$. Since $f(z_1)), f(z_2) \in F_{s_0}$, Lemma \ref{autlem20} implies that $m\in \aut_{s_0}(G)$. Consequently, by Lemma \ref{autlem40}
\[
f((m\circ m)(z_1)) = \gamma_m(f(z_1)) =f(z_2)
\]
which implies that
\[
z_2 = (m \circ m) (z_1).
\]
Now, as $m\in \aut_{s_0}(G)$, Definition \ref{autdef30} implies that
\[
\Gamma(m) (e(z)) = e((m\circ m) (z)),\qquad z \in \d.
\]
Consequently,
\[
\Gamma(m) (e(z_1)) = e((m\circ m) (z_1)) =e(z_2),
\]
which implies \eqref{aut150}. This completes the proof  that $\Lambda$ is well defined. Also observe that \eqref{aut120} and \eqref{aut130} together imply that
\be\label{aut160}
\Lambda (\gamma_m(s)) = \Gamma(m) \Lambda(s)
\ee
for all $s\in G$ and also that
\be\label{aut170}
\Lambda (f(z)) = e(z)
\ee
for all $z\in \d$. In particular, $\Lambda(s_0) =d_0$.

Now fix a general point $r(z)$ on the royal geodesic. If we choose $m$ so that $m(z_0)=z$, then it follows that
\begin{align*}
&\ \ \ \ \Lambda(r(z))\\
&= \Lambda(r(m(z_0)))\\
\eqref{aut44}\qquad\qquad&=\Lambda(\gamma_m (r(z_0)))\\
\eqref{aut160} \text{ and } s_0=r(z_0)\qquad\qquad&=\Gamma(m) \Lambda(s_0)\\
&=\Gamma(m) d_0\\
&=\Gamma(m)d(z_0)\\
\eqref{aut50}\qquad\qquad&=d(m(z_0))\\
&=d(z),
\end{align*}
i.e.,
\be\label{aut180}
\Lambda(r(z)) = d(z),\qquad z \in \d.
\ee

Now fix $z_1 \in \d$ and choose $m$ so that $m(z_0) = z_1$. Since $\gamma_m(r(z_0)) = r(z_1)$, Lemma \ref{autlem20} implies that
\[
\gamma_m(F_{r(z_0)})=F_{r(z_1)},
\]
and since $\Gamma(m) d(z_0) =d(z_1)$, Condition (iii) in Definition \ref{autdef30} implies that
\[
\Gamma(m)(E_{d(z_0)})=E_{d(z_1)}.
\]
Therefore,
\begin{align*}
\Lambda(F_{r(z_1)}) &= \Lambda(\gamma_m(F_{r(z_0)}))\\
&=\Gamma (m) \Lambda (F_{r(z_0)}))\\
&=\Gamma(m) E_{d(z_0)}\\
&=E_{d(z_1)}.
\end{align*}
Summarizing, we have shown that if $\cale$ denotes the partition of Lemma \ref{autlem10} and $\calf$ denotes the partition of Definition \ref{autdef30}, then $\Lambda$ induces a map
\[
\calf \ni F_{r(z)} \overset{\Lambda^\sim}{\mapsto} E_{d(z)} \in \cale.
\]
Furthermore, as the map
\[
R \ni r(z) \mapsto d(z) \in D
\]
is a bijection, so also $\Lambda^\sim$ is a bijection.

Note that since $\Lambda^\sim$ is a bijection, it follows immediately that $\Lambda$ is surjective. Also, to prove that $\Lambda$ is 1-1, it suffices to show that $\Lambda$ is injective on each flat geodesic. But if $m$ and $z_1$ are as in the previous paragraph, then
\be\label{aut190}
\Lambda| F_{r(z_1)} = \Gamma (m) \circ e \circ f^{-1} \circ \gamma_m^{-1}
\ee
is 1-1.

There remains to prove that $\Lambda$ and $\Lambda^{-1}$ are holomorphic. Fix $s\in G$ and let $X=(d\Lambda) _s$ viewed as a real linear mapping from $\c^2$ to $\c^2$. Note first that \eqref{aut190} implies that 
\be\label{aut200}
\forall_{s\in G}\ \ X(s^\flat) = (\Lambda (s))^\flat \text{ and } X|s^\flat \text{ is complex linear}.
 \ee
 Next, observe that if $r\in \r$, $\alpha \in \c$, and $s\in G$, then
\begin{align*}
X(v_{r,\alpha} (s))&= d\Lambda (v_{r,\alpha} (s))\\
\eqref{aut92}\qquad\qquad &= d\Lambda \big(\frac{d}{dt}\gamma_{m_{r,\alpha} (t)} (s) |_{t=0}\big)\\
\text{chain rule}\qquad\qquad &=\frac{d}{dt}\ \big(\Lambda \circ \gamma_{m_{r,\alpha} (t)}\big) (s)\ \big|_{t=0}\\
\eqref{aut160}\qquad\qquad &=\frac{d}{dt}\ \big(\Gamma (m_{r,\alpha} (t))\circ \Lambda \big) (s)\ \big|_{t=0}\\
&= \frac{d}{dt}( \Gamma(m_{r,\alpha} (t))(\Lambda(s)))\big|_{t=0}\\
\eqref{aut106}\qquad\qquad &=w_{r,\alpha}(\Lambda(s))\\
\eqref{aut114}\qquad\qquad &=\big(\frac{d\Gamma}{d\gamma}\big)_{s,\Lambda(s)}(v_{r,\alpha}(s))
\end{align*}
In particular, if we let $s=f(z)$, then \eqref{aut170} implies that
\[
X(v_{r,\alpha} (f(z))) = \big(\frac{d\Gamma}{d\gamma}\big)_{f(z),e(z)}(v_{r,\alpha}(f(z)))
\]
for all $z\in \d$, $r\in \r$, and $\alpha \in \c$. But $\aut{\Omega}$ acts sharply on $\Omega$, so that
\[
\big(\frac{d\Gamma}{d\gamma}\big)_{f(z),e(z)}(f(z)^\sharp) = e(z)^\sharp \text{ and } \big(\frac{d\Gamma}{d\gamma}\big)_{f(z),e(z)}\big|f(z)^\sharp \text{ is complex linear}
\]
for all $z\in \d$. Hence,
\[
\forall_{z\in\d}\ \ X(f(z)^\sharp) = e(z)^\sharp \text{ and } X |f(z)^\sharp\text{ is complex linear}
\]
which implies via \eqref{aut160} and Propositions \eqref{autprop40} and \eqref{autprop50} that
\be\label{aut210}
\forall_{s \in G}\ \ X (s^\sharp) = (\Lambda(s))^\sharp \text{ and } X |s^\sharp\text{ is complex linear}.
\ee
Recalling that $X:\c^2\to \c^2$ is real linear, it follows from \eqref{aut200}, \eqref{aut210}, and the linear independence of $s^\flat$ and $s^\sharp$ that $X$ is complex linear. Therefore, since $X=d\Lambda$, $\Lambda$ is differentiable at $s$. Since $\Lambda(s)^\flat$ and $\Lambda(s)^\sharp$ are linearly independent, it follows that $d\Lambda$ is nonsingular. Hence, by the open mapping theorem, $\Lambda^{-1}$ is holomorphic as well. 
\end{proof}

